Post-Hoc Domain Adaptation via Guided Data Homogenization

Addressing shifts in data distributions is an important prerequisite for the deployment of deep learning models to real-world settings. A general approach to this problem involves the adjustment of models to a new domain through transfer learning. However, in many cases, this is not applicable in a post-hoc manner to deployed models and further parameter adjustments jeopardize safety certifications that were established beforehand. In such a context, we propose to deal with changes in the data distribution via guided data homogenization which shifts the burden of adaptation from the model to the data. This approach makes use of information about the training data contained implicitly in the deep learning model to learn a domain transfer function. This allows for a targeted deployment of models to unknown scenarios without changing the model itself. We demonstrate the potential of data homogenization through experiments on the CIFAR-10 and MNIST data sets.

==> graphs/evaluation.tex <==
\begin{tikzpicture}[node distance=1cm and 1.7cm, auto]

\node (A) [node, fill=red!7] {\textbf{target} \\ $\set A$};
\node (B) [node, below= of A] {\textbf{original} \\ $\set B_\text{true}$};
\node (C) [node, below= 2.2cm of B, fill=blue!0] {\textbf{validation} \\ $\set C_{true}$};

\node (Bp) [node, right= of B, fill=blue!2] {perturbed \\ \textbf{source} \\ $\set B$};
\node (Br) [node, right= of Bp, fill=blue!7] {\textbf{reconstructed} \\ $\rho^* (\set B)$};


\draw [arrow, dashed, thin] (B) -- (Bp) node (Pert) [midway, function, dashed] {$\delta$};
\draw [arrow] (Bp) -- (Br) node (Rec) [midway, function] {$\rho^*$};
\node [fill=white, below= 0cm of Pert] {\footnotesize \textit{unknown}};
\node [fill=white, below= 0cm of Rec] {\footnotesize \textit{learned}};


\node (Net) [function, fill=gray!5, above= of Br] {neural \\ network};
\node (vNet) [function, fill=gray!5, right= of Net] {verification \\ neural \\ network};

\draw [arrow, Mahogany, thin, bend left=20] (A) to (Net);
\draw [arrow, Mahogany, thin, bend left=20] (A) to node[below] {\footnotesize trained} (vNet);
\draw [arrow, Blue, thin] (Net.210) to[bend right=20] node [midway, above, sloped] {\footnotesize optimized} (Rec.north);

\node (Cp) [node, right= of C, fill=blue!0] {\textbf{perturbed} \\ $ {\set C}$};
\node (Cr) [node, right= of Cp, fill=blue!0] {\textbf{reconstructed} \\ $\rho ^*( {\set C})$};


\draw [arrow, dashed, thin] (C) -- (Cp);
\draw [arrow] (Cp) -- (Cr);

\draw [arrow, dashed, thin] (C) -- (Cp) node (Pert) [midway, function, dashed] {$\delta$};
\draw [arrow] (Cp) -- (Cr) node (Rec) [midway, function] {$\rho^*$};

\draw [arrow, <->, thin, OliveGreen] (Br.south) to [rect connect h=-0.75cm] (B.south);
\draw [arrow, <->, thin, OliveGreen] (Cr.north) to [rect connect h=0.75cm] (C.north);

\path (Br.east) to [out=0, in=270]  node [near end, OliveGreen, xshift=0.1cm] {accuracy} (vNet.265);
\draw [arrow, thin, OliveGreen] (Br.east) to [out=0, in=320] (Net.315);
\draw [arrow, thin, OliveGreen] (Cr.east) to [out=0, in=320] (Net.325);
\draw [arrow, thin, OliveGreen] (Cr.east) to [out=0, in=270] (vNet.south);


\node [OliveGreen] at ($(Bp)!0.5!(Cp)$) {IQA metrics};

\node [below= 1.5cm of Pert] (Id) {$\vec I$};
\path (Id) -| node[anchor=center] (Idr) {$\widehat {\vec I}$} (Rec);
\draw [arrow] (Id) -- 
node[near start, xshift=0.2cm, function] {$\delta$} 
node[near end, xshift=-0.2cm, function] {$\rho^*$} (Idr);
\draw [arrow, <->, thin, OliveGreen] (Idr.south) to [rect connect h=-0.6cm] (Id.south);
\node [OliveGreen, yshift=-1.2cm] at ($(Id)!0.5!(Idr)$) {rel. error};
% \node [circle, fill=blue] at (Idr){};
% \draw (0,0)|-node{mid}(2,3);
% \node [below= 1cm of Rec] {};
% \node (Cbelow) [below= of Cp] {EEE};
% \draw [arrow, dashed, thin] (C) -- (Cp) node (Pert) [midway, function, dashed] {$\delta$};
% \draw [arrow] (Cp) -- (Cr) node (Rec) [midway, function] {$\rho^*$};

\end{tikzpicture}
